The Fake News Effect: Experimentally Identifying Motivated Reasoning Using Trust in News

Motivated reasoning posits that people distort how they process information in the direction of beliefs they find attractive. This paper creates a novel experimental design to identify motivated reasoning from Bayesian updating when people have preconceived beliefs. It analyzes how subjects assess the veracity of information sources that tell them the median of their belief distribution is too high or too low. Bayesians infer nothing about the source veracity, but motivated beliefs are evoked. Evidence supports politically-motivated reasoning about immigration, income mobility, crime, racial discrimination, gender, climate change, and gun laws. Motivated reasoning helps explain belief biases, polarization, and overconfidence.

==> change_guess.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
Pro-Party News      &    0.122&         &    0.114&         &         &    0.024\\
                    &  (0.019)&         &  (0.020)&         &         &  (0.017)\\
polarizing          &         &    0.061&    0.032&         &   -0.017&   -0.022\\
                    &         &  (0.018)&  (0.018)&         &  (0.015)&  (0.015)\\
P(True)             &         &         &         &    1.134&    1.139&    1.131\\
                    &         &         &         &  (0.057)&  (0.057)&  (0.059)\\
Question FE         &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Subject FE          &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations        &     4085&     4085&     4085&     4085&     4085&     4085\\
\(R^{2}\)           &     0.28&     0.28&     0.28&     0.45&     0.45&     0.45\\
Mean                &    0.658&    0.658&    0.658&    0.658&    0.574&    0.574\\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> estimated_motives.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &Hyp. direction         &Pro-R vs. Pro-D         &Diff. by prior         \\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\hline
Climate topic       &    0.083&    0.068&    0.085\\
                    &  (0.010)         &  (0.019)         &  (0.009)         \\
Race topic          &    0.075&    0.029         &    0.059\\
                    &  (0.019)         &  (0.041)         &  (0.009)         \\
Mobility topic      &    0.032&    0.039&    0.021\\
                    &  (0.005)         &  (0.011)         &  (0.005)         \\
Refugees topic      &    0.010&    0.017&    0.004 \\
                    &  (0.002)         &  (0.005)         &  (0.002)         \\
Obama crime topic   &    0.026&    0.043&    0.009  \\
                    &  (0.006)         &  (0.013)         &  (0.005)         \\
Gender topic        &    0.605&    0.534         &    0.279  \\
                    &  (0.192)         &  (0.413)         &  (0.149)         \\
Gun laws topic      &    0.003 &    0.001         &    0.002         \\
                    &  (0.001)         &  (0.003)         &  (0.001)         \\
Media topic         &    0.001         &    0.018  &    0.020\\
                    &  (0.004)         &  (0.009)         &  (0.004)         \\
Rep score topic     &    0.029&    0.073&    0.021\\
                    &  (0.006)         &  (0.014)         &  (0.007)         \\
Dem score topic     &    0.032&    0.050&    0.025\\
                    &  (0.007)         &  (0.014)         &  (0.007)         \\
Own performance topic    &    0.007 &                  &    0.016\\
              &  (0.003)         &                  &  (0.004)         \\
Question FE         &       No         &      Yes         &      Yes         \\
\hline
Observations        &     8785         &     7902         &     8785         \\
\(R^{2}\)           &     0.01         &     0.03         &     0.03         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> fne_change_guess_replication.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
Pro-Party News      &    0.122&         &    0.114&         &         &    0.024\\
                    &  (0.019)&         &  (0.020)&         &         &  (0.017)\\
polarizing          &         &    0.061&    0.032&         &   -0.017&   -0.022\\
                    &         &  (0.018)&  (0.018)&         &  (0.015)&  (0.015)\\
P(True)             &         &         &         &    1.134&    1.139&    1.131\\
                    &         &         &         &  (0.057)&  (0.057)&  (0.059)\\
Question FE         &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Subject FE          &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
\hline
Observations        &     4085&     4085&     4085&     4085&     4085&     4085\\
\(R^{2}\)           &     0.28&     0.28&     0.28&     0.45&     0.45&     0.45\\
Mean                &    0.658&    0.658&    0.658&    0.658&    0.574&    0.574\\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> heterogeneity_direction_horserace_paper.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{9}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         &\multicolumn{1}{c}{ (9) }         \\
\hline
Rep News x Pro-Rep  &     0.13&                  &                  &                  &                  &                  &                  &                  &     0.12\\
                    &     (0.01)         &                  &                  &                  &                  &                  &                  &                  &   (0.01)         \\
Rep News x (Age$>$32) &                  &     0.00         &                  &                  &                  &                  &                  &                  &    -0.01         \\
                    &                  &   (0.01)         &                  &                  &                  &                  &                  &                  &  (0.01)         \\
Rep News x Male     &                  &                  &     0.00         &                  &                  &                  &                  &                  &     0.00         \\
                    &                  &                  &   (0.01)         &                  &                  &                  &                  &                  &   (0.01)         \\
Rep News x White    &                  &                  &                  &     0.03  &                  &                  &                  &                  &     0.02        \\
                    &                  &                  &                  &   (0.02)         &                  &                  &                  &                  &   (0.02)         \\
Rep News x College  &                  &                  &                  &                  &     0.01         &                  &                  &                  &     0.02        \\
                    &                  &                  &                  &                  &   (0.01)         &                  &                  &                  &    (0.01)         \\
Rep News x (Inc$>$50K)&                  &                  &                  &                  &                  &    -0.01         &                  &                  &    -0.02         \\
                    &                  &                  &                  &                  &                  &   (0.01)         &                  &                  &   (0.01)         \\
Rep News x Red State&                  &                  &                  &                  &                  &                  &     0.02  &                  &     {0.01}         \\
                    &                  &                  &                  &                  &                  &                  &   (0.01)         &                  &   (0.01)         \\
Rep News x Religious&                  &                  &                  &                  &                  &                  &                  &     0.05&     0.02         \\
                    &                  &                  &                  &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
Rep News            &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
Question FE         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
Round FE            &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
Observations        &     7902         &     7902         &     7902         &     7902         &     7902         &     7902         &     7902         &     7902         &     7902         \\
\(R^{2}\)           &     0.26         &     0.25         &     0.25         &     0.25         &     0.25         &     0.25         &     0.25         &     0.25         &     0.26         \\
Mean                &     0.57         &     0.57         &     0.57         &     0.57         &     0.57         &     0.57         &     0.57         &     0.57         &     0.57         \\
\hline\hline
\multicolumn{10}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> heterogeneity_magnitude_horserace.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{9}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         &\multicolumn{1}{c}{(9)}         \\
\hline
Pro-Motive x Pro-R &     0.06&                  &                  &                  &                  &                  &                  &                  &     0.08\\
x Partisan            &   (0.02)         &                  &                  &                  &                  &                  &                  &                  &   (0.03)         \\
Pro-Motive x Pro-R &    -0.02         &                  &                  &                  &                  &                  &                  &                  &     0.00         \\
x Moderate            &   (0.01)         &                  &                  &                  &                  &                  &                  &                  &   (0.03)         \\
Pro-Motive x Pro-D &     0.11&                  &                  &                  &                  &                  &                  &                  &     0.12\\
x Moderate            &   (0.01)         &                  &                  &                  &                  &                  &                  &                  &   (0.02)         \\
Pro-Motive x Pro-D &     0.13&                  &                  &                  &                  &                  &                  &                  &     0.14\\
x Partisan            &   (0.01)         &                  &                  &                  &                  &                  &                  &                  &   (0.02)         \\
Pro-Motive x (Age$>$32) &                  &     0.00         &                  &                  &                  &                  &                  &                  &     0.01         \\
                 &                  &   (0.01)         &                  &                  &                  &                  &                  &                  &   (0.01)         \\
Pro-Motive x Male   &                  &                  &     0.00         &                  &                  &                  &                  &                  &     0.01         \\
                    &                  &                  &   (0.01)         &                  &                  &                  &                  &                  &   (0.01)         \\
Pro-Motive x White  &                  &                  &                  &    -0.02         &                  &                  &                  &                  &    -0.01         \\
                    &                  &                  &                  &   (0.01)         &                  &                  &                  &                  &   (0.01)         \\
Pro-Motive x College&                  &                  &                  &                  &     0.01         &                  &                  &                  &     0.01         \\
                    &                  &                  &                  &                  &   (0.01)         &                  &                  &                  &   (0.01)         \\
Pro-Motive x (Inc$>$50K)        &                  &                  &                  &                  &                  &    -0.02 &                  &                  &    -0.02  \\
          &                  &                  &                  &                  &                  &   (0.01)         &                  &                  &   (0.01)         \\
Pro-Motive x Red State       &                  &                  &                  &                  &                  &                  &    -0.02  &                  &    -0.01         \\
           &                  &                  &                  &                  &                  &                  &   (0.01)         &                  &   (0.01)         \\
Pro-Motive x Religious          &                  &                  &                  &                  &                  &                  &                  &    -0.04&    -0.01         \\
        &                  &                  &                  &                  &                  &                  &                  &   (0.01)         &   (0.01)         \\
Pro-Motive News     &       No         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &       No         \\
Question FE         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
Round FE            &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
Observations        &     8793         &     8793         &     8793         &     8793         &     8793         &     8793         &     8793         &     8793         &     8793         \\
\(R^{2}\)           &     0.24         &     0.23         &     0.23         &     0.23         &     0.23         &     0.23         &     0.23         &     0.23         &     0.24         \\
Mean                &     0.58         &     0.58         &     0.58         &     0.58         &     0.58         &     0.58         &     0.58         &     0.58         &     0.58         \\
\hline\hline
\multicolumn{10}{l}{Standard errors in parentheses}\\
\end{tabular}
}


==> moreas_heterogeneity.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Relative party preference predicts motivated reasoning across all topics}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         &\multicolumn{1}{c}{(8)}         \\
\hline
Male                &    0.083\sym{***}&                  &                  &                  &                  &                  &                  &                  \\
                    &  (0.009)         &                  &                  &                  &                  &                  &                  &                  \\
Female              &    0.096\sym{***}&                  &                  &                  &                  &                  &                  &                  \\
                    &  (0.010)         &                  &                  &                  &                  &                  &                  &                  \\
Age > 33            &                  &    0.089\sym{***}&                  &                  &                  &                  &                  &                  \\
                    &                  &  (0.010)         &                  &                  &                  &                  &                  &                  \\
Age <= 33           &                  &    0.088\sym{***}&                  &                  &                  &                  &                  &                  \\
                    &                  &  (0.009)         &                  &                  &                  &                  &                  &                  \\
White               &                  &                  &    0.083\sym{***}&                  &                  &                  &                  &                  \\
                    &                  &                  &  (0.007)         &                  &                  &                  &                  &                  \\
Nonwhite            &                  &                  &    0.105\sym{***}&                  &                  &                  &                  &                  \\
                    &                  &                  &  (0.014)         &                  &                  &                  &                  &                  \\
Income > 50K        &                  &                  &                  &    0.078\sym{***}&                  &                  &                  &                  \\
                    &                  &                  &                  &  (0.010)         &                  &                  &                  &                  \\
Income < 50K        &                  &                  &                  &    0.098\sym{***}&                  &                  &                  &                  \\
                    &                  &                  &                  &  (0.009)         &                  &                  &                  &                  \\
College             &                  &                  &                  &                  &    0.088\sym{***}&                  &                  &                  \\
                    &                  &                  &                  &                  &  (0.008)         &                  &                  &                  \\
No College          &                  &                  &                  &                  &    0.088\sym{***}&                  &                  &                  \\
                    &                  &                  &                  &                  &  (0.011)         &                  &                  &                  \\
High Quiz Score     &                  &                  &                  &                  &                  &    0.109\sym{***}&                  &                  \\
                    &                  &                  &                  &                  &                  &  (0.009)         &                  &                  \\
Low Quiz Score      &                  &                  &                  &                  &                  &    0.071\sym{***}&                  &                  \\
                    &                  &                  &                  &                  &                  &  (0.009)         &                  &                  \\
Partisan            &                  &                  &                  &                  &                  &                  &    0.112\sym{***}&                  \\
                    &                  &                  &                  &                  &                  &                  &  (0.009)         &                  \\
Moderate            &                  &                  &                  &                  &                  &                  &    0.064\sym{***}&                  \\
                    &                  &                  &                  &                  &                  &                  &  (0.010)         &                  \\
good\_news\_long      &                  &                  &                  &                  &                  &                  &                  &    0.080\sym{***}\\
                    &                  &                  &                  &                  &                  &                  &                  &  (0.009)         \\
good\_news\_short     &                  &                  &                  &                  &                  &                  &                  &    0.098\sym{***}\\
                    &                  &                  &                  &                  &                  &                  &                  &  (0.008)         \\
Question FE         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
Round FE            &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
Observations        &     7902         &     7902         &     7902         &     7902         &     7902         &     7902         &     7902         &     7902         \\
\(R^{2}\)           &     0.25         &     0.25         &     0.25         &     0.25         &     0.25         &     0.25         &     0.25         &     0.25         \\
Mean                &    0.573         &    0.573         &    0.573         &    0.573         &    0.573         &    0.573         &    0.573         &    0.573         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{9}{l}{\footnotesize OLS, errors clustered at subject level. Adjusted for good-and-bad-news-weighted FE.}\\
\multicolumn{9}{l}{\footnotesize \sym{+} \(p<0.10\), \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.005\)}\\
\end{tabular}
\end{table}


==> moreas_political_only7to12.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
Pro-Party News      &    0.095&    0.090&    0.045&    0.040&         &    0.078\\
                    &  (0.009)&  (0.010)&  (0.019)&  (0.009)&         &  (0.010)\\
Partisanship x      &         &         &    0.096&         &         &         \\
Pro-Party           &         &         &  (0.033)&         &         &         \\
Anti-Party News     &         &         &         &   -0.046&         &         \\
                    &         &         &         &  (0.010)&         &         \\
True News           &         &         &         &         &   -0.067&   -0.044\\
                    &         &         &         &         &  (0.010)&  (0.010)\\
Question FE         &      Yes&      Yes&      Yes&       No&      Yes&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Subject FE          &       No&      Yes&      Yes&      Yes&      Yes&      Yes\\
Subject controls    &      Yes&       No&       No&       No&       No&       No\\
Neutral News        &       No&       No&       No&      Yes&       No&       No\\
\hline
Observations        &     3485&     3484&     3484&     4737&     3484&     3484\\
\(R^{2}\)           &     0.04&     0.37&     0.37&     0.30&     0.36&     0.37\\
Mean                &    0.586&    0.586&    0.586&    0.587&    0.586&    0.586\\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> moreas_political_onlyfirst6.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
\hline
Pro-Party News      &    0.081&    0.077&    0.046&    0.030&         &    0.069\\
                    &  (0.009)&  (0.009)&  (0.018)&  (0.009)&         &  (0.010)\\
Partisanship x      &         &         &    0.063&         &         &         \\
Pro-Party           &         &         &  (0.033)&         &         &         \\
Anti-Party News     &         &         &         &   -0.045&         &         \\
                    &         &         &         &  (0.009)&         &         \\
True News           &         &         &         &         &   -0.046&   -0.024\\
                    &         &         &         &         &  (0.010)&  (0.010)\\
Question FE         &      Yes&      Yes&      Yes&       No&      Yes&      Yes\\
Round FE            &      Yes&      Yes&      Yes&      Yes&      Yes&      Yes\\
Subject FE          &       No&      Yes&      Yes&      Yes&      Yes&      Yes\\
Subject controls    &      Yes&       No&       No&       No&       No&       No\\
Neutral News        &       No&       No&       No&      Yes&       No&       No\\
\hline
Observations        &     3521&     3521&     3521&     4919&     3521&     3521\\
\(R^{2}\)           &     0.04&     0.36&     0.36&     0.28&     0.35&     0.36\\
Mean                &    0.563&    0.563&    0.563&    0.564&    0.563&    0.563\\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> moreas_political_prevgood.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
Previous Pro-Party  &   -0.001         &   -0.001         &   -0.002         &   -0.002         \\
                    &  (0.002)         &  (0.002)         &  (0.002)         &  (0.002)         \\
Pro-Party News      &    0.087&    0.039&    0.036&    0.076\\
                    &  (0.007)         &  (0.013)         &  (0.007)         &  (0.007)         \\
Partisanship x Pro-Party     &                  &    0.050&                  &                  \\
           &                  &  (0.012)         &                  &                  \\
Anti-Party News     &                  &                  &   -0.048&                  \\
                    &                  &                  &  (0.007)         &                  \\
True News           &                  &                  &                  &   -0.034\\
                    &                  &                  &                  &  (0.007)         \\
Neutral News        &       No         &       No         &      Yes         &       No         \\
Question FE         &      Yes         &      Yes         &       No         &      Yes         \\
Round FE            &      Yes         &      Yes         &      Yes         &      Yes         \\
Subject FE          &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
Observations        &     7902         &     7902         &    10552         &     7902         \\
\(R^{2}\)           &     0.25         &     0.25         &     0.21         &     0.25         \\
Mean                &    0.573         &    0.573         &    0.574         &    0.573         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> moreas_political_replication.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
Pro-Party News      &    0.053&    0.010         &                  &    0.046\\
                    &  (0.009)         &  (0.018)         &                  &  (0.009)         \\
Partisanship x      &                  &    0.044&                  &                  \\
Pro-Party           &                  &  (0.016)         &                  &                  \\
True News           &                  &                  &   -0.043&   -0.033\\
                    &                  &                  &  (0.009)         &  (0.009)         \\
Question FE         &      Yes         &      Yes         &      Yes         &      Yes         \\
Round FE            &      Yes         &      Yes         &      Yes         &      Yes         \\
Subject FE          &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
Observations        &     5314         &     5314         &     5314         &     5314         \\
\(R^{2}\)           &     0.32         &     0.32         &     0.32         &     0.33         \\
Mean                &    0.578         &    0.578         &    0.578         &    0.578         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> moreas_yaib.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
Unskewed            &   -0.011         &   -0.003         &   -0.019  &    0.002         \\
                    &  (0.010)         &  (0.014)         &  (0.011)         &  (0.013)         \\
Pro-Party News      &    0.084&    0.041&    0.028&    0.075\\
                    &  (0.008)         &  (0.015)         &  (0.008)         &  (0.008)         \\
Unskewed x Pro-Party&    0.014         &   -0.002         &    0.021         &    0.006         \\
                    &  (0.013)         &  (0.024)         &  (0.014)         &  (0.013)         \\
Partisanship x Pro-Party     &                  &    0.044&                  &                  \\
           &                  &  (0.014)         &                  &                  \\
Unskewed x Partisanship x Pro-Party        &                  &    0.017         &                  &                  \\
&                  &  (0.022)         &                  &                  \\
Anti-Party News     &                  &                  &   -0.052&                  \\
                    &                  &                  &  (0.008)         &                  \\
Unskewed x Anti-Party         &                  &                  &    0.006         &                  \\
          &                  &                  &  (0.014)         &                  \\
True News           &                  &                  &                  &   -0.027\\
                    &                  &                  &                  &  (0.008)         \\
Unskewed x True News&                  &                  &                  &   -0.021         \\
                    &                  &                  &                  &  (0.014)         \\
Neutral News        &       No         &       No         &      Yes         &       No         \\
Question FE         &      Yes         &      Yes         &       No         &      Yes         \\
Round FE            &      Yes         &      Yes         &      Yes         &      Yes         \\
Subject FE          &      Yes         &      Yes         &      Yes         &      Yes         \\
\hline
Observations        &     7902         &     7902         &    10552         &     7902         \\
\(R^{2}\)           &     0.25         &     0.25         &     0.21         &     0.25         \\
Mean                &    0.573         &    0.573         &    0.574         &    0.573         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> news_assessment_scores.tex <==
\begin{tabular}{l*{3}{c}}
\hline\hline
                                   &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
Politicized Topic                  &    -4.14&    -1.92&    -1.92\\
                                   &   (0.60)&   (1.03)&   (1.03)\\
Partisanship x Politicized Topic   &         &    -5.09&    -3.58\\
                                   &         &   (1.89)&   (1.14)\\
Partisanship x Neutral Topic       &         &         &     1.53\\
                                   &         &         &   (1.62)\\
Round FE                           &      Yes&      Yes&      Yes\\
Subject FE                         &      Yes&      Yes&       No\\
\hline
Observations                       &    11612&    11612&    11612\\
\(R^{2}\)                          &     0.12&     0.12&     0.01\\
Mean                               &    66.83&    66.83&    66.83\\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> news_points.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{{l}@{\hspace{18mm}}{c}@{\hspace{8mm}}{c}@{\hspace{8mm}}{c}}
\hline\hline
                    &\multicolumn{1}{c}{\hspace{-8mm} (1)}         &\multicolumn{1}{c}{\hspace{-8mm} (2)}         &\multicolumn{1}{c}{(3)}         \\
\hline
Politicized Topic Indicator  &   -4.14&   -1.92  &   -1.92  \\
                    &  (0.62)         &  (1.08)         &  (1.03)         \\
Partisanship x Politicized Topic Indicator    &                  &   -5.09 &   -3.58\\
       &                  &  (1.98)         &  (1.14)         \\
Partisanship x Neutral Topic Indicator    &                  &                  &    1.53         \\
             &                  &                  &  (1.62)         \\
Round FE            &      Yes         &      Yes         &      Yes         \\
Subject FE          &      Yes         &      Yes         &       No         \\
\hline
Observations        &    11612         &    11612         &    11612         \\
\(R^{2}\)           &     0.12         &     0.12         &     0.01         \\
Mean                &   69.47         &   69.47         &   69.47         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> overconfidence_moreas.tex <==
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
\hline
Pro-Performance     &    0.055&    0.056\\
                    &  (0.016)&  (0.016)\\
Overconfidence\hspace{30mm}&   -0.015&   -0.009\\
                    &  (0.038)&  (0.037)\\
Pro-Performance x Overconfidence  &    0.114&    0.119\\
      &  (0.057)&  (0.056)\\
Controls            &       No&      Yes\\
\hline
Observations        &      980&      980\\
\(R^{2}\)           &     0.02&     0.04\\
Mean                &    0.600&    0.600\\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> overplacement.tex <==
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{News Pts}&\multicolumn{1}{c}{ }&\multicolumn{1}{c}{Performance}&\multicolumn{1}{c}{ }&\multicolumn{1}{c}{Expectation}&\multicolumn{1}{c}{ }\\
\hline
Partisanship        &    -3.58&    -3.59&    -4.74&    -4.64&     6.13&     7.95\\
                    &   (1.14)&   (1.15)&   (2.60)&   (2.67)&   (2.18)&   (2.15)\\
Subject controls    &       No&      Yes&       No&      Yes&       No&      Yes\\
\hline
Observations        &     8696&     8696&      987&      987&      987&      987\\
\(R^{2}\)           &     0.02&     0.02&     0.00&     0.03&     0.01&     0.13\\
Mean                &    65.86&    65.86&    47.64&    47.64&    50.36&    50.36\\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> overprecision_fake_news.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
True News           &   -0.061\sym{***}&   -0.058\sym{***}&   -0.058\sym{***}&   -0.056\sym{***}\\
                    &  (0.006)         &  (0.006)         &  (0.006)         &  (0.006)         \\
Overprecision       &                  &    0.030\sym{***}&                  &    0.025\sym{***}\\
                    &                  &  (0.008)         &                  &  (0.008)         \\
Overprecision x True News &                  &   -0.057\sym{***}&                  &   -0.057\sym{***}\\
               &                  &  (0.011)         &                  &  (0.011)         \\
Question FE         &      Yes         &      Yes         &      Yes         &      Yes         \\
Round FE            &      Yes         &      Yes         &      Yes         &      Yes         \\
Subject FE          &       No         &       No         &      Yes         &      Yes         \\
\hline
Observations        &     8696         &     8696         &     8696         &     8696         \\
\(R^{2}\)           &     0.02         &     0.03         &     0.23         &     0.23         \\
Mean                &    0.573         &    0.573         &    0.573         &    0.573         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize OLS, errors clustered at subject level.}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> overprecision_miscalibration.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\hline
Partisanship x      &     0.08\sym{***}&     0.07\sym{***}\\
Political           &   (0.02)         &   (0.02)         \\
Partisanship x      &     0.02         &     0.01         \\
Neutral             &   (0.03)         &   (0.03)         \\
Log(Size of CI) x   &                  &    -0.10\sym{***}\\
Political           &                  &   (0.01)         \\
Log(Size of CI) x   &                  &    -0.22\sym{***}\\
Neutral             &                  &   (0.01)         \\
Question FE         &      Yes         &      Yes         \\
Round FE            &      Yes         &      Yes         \\
\hline
Observations        &    11844         &    11767         \\
\(R^{2}\)           &     0.14         &     0.20         \\
Mean                &    -0.00         &    -0.00         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize OLS, errors clustered at subject level.}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> overprecision_party_replication.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
\hline
Partisanship \hspace{10mm}        &    0.055  &    0.055  \\
                    &  (0.030)         &  (0.030)         \\
Subject controls  \hspace{10mm}    &       No         &      Yes         \\
\hline
Observations        &     5314         &     5314         \\
\(R^{2}\)           &     0.00         &     0.01         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> structural_motives.tex <==
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
Climate topic       &    0.073&         &         \\
                    &  (0.009)&         &         \\
Race topic          &    0.073&         &         \\
                    &  (0.019)&         &         \\
Mobility topic      &    0.031&         &         \\
                    &  (0.005)&         &         \\
Refugees topic      &    0.010&         &         \\
                    &  (0.002)&         &         \\
Obama crime topic   &    0.026&         &         \\
                    &  (0.006)&         &         \\
Gender topic        &    0.595&         &         \\
                    &  (0.182)&         &         \\
Gun laws topic      &    0.002&         &         \\
                    &  (0.001)&         &         \\
Media topic         &    0.000&         &         \\
                    &  (0.004)&         &         \\
Rep score topic     &    0.028&         &         \\
                    &  (0.006)&         &         \\
Dem score topic     &    0.032&         &         \\
                    &  (0.006)&         &         \\
Own performance     &    0.007&         &         \\
topic               &  (0.003)&         &         \\
Climate topic       &         &    0.058&         \\
                    &         &  (0.017)&         \\
Race topic          &         &    0.031&         \\
                    &         &  (0.040)&         \\
Mobility topic      &         &    0.037&         \\
                    &         &  (0.010)&         \\
Refugees topic      &         &    0.016&         \\
                    &         &  (0.004)&         \\
Obama crime topic   &         &    0.044&         \\
                    &         &  (0.012)&         \\
Gender topic        &         &    0.511&         \\
                    &         &  (0.390)&         \\
Gun laws topic      &         &    0.001&         \\
                    &         &  (0.002)&         \\
Media topic         &         &    0.015&         \\
                    &         &  (0.009)&         \\
Rep score topic     &         &    0.069&         \\
                    &         &  (0.014)&         \\
Dem score topic     &         &    0.051&         \\
                    &         &  (0.013)&         \\
Climate topic       &         &         &    0.076\\
                    &         &         &  (0.007)\\
Race topic          &         &         &    0.057\\
                    &         &         &  (0.008)\\
Mobility topic      &         &         &    0.019\\
                    &         &         &  (0.005)\\
Refugees topic      &         &         &    0.006\\
                    &         &         &  (0.001)\\
Obama crime topic   &         &         &    0.010\\
                    &         &         &  (0.004)\\
Gender topic        &         &         &    0.234\\
                    &         &         &  (0.129)\\
Gun laws topic      &         &         &    0.001\\
                    &         &         &  (0.001)\\
Media topic         &         &         &    0.018\\
                    &         &         &  (0.004)\\
Rep score topic     &         &         &    0.022\\
                    &         &         &  (0.006)\\
Dem score topic     &         &         &    0.024\\
                    &         &         &  (0.006)\\
Own performance     &         &         &    0.013\\
topic               &         &         &  (0.003)\\
Question FE         &       No&      Yes&      Yes\\
\hline
Observations        &     8765&     7882&     8765\\
\(R^{2}\)           &     0.01&     0.03&     0.03\\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> structural_motives_paper.tex <==
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Hyp. direction}&\multicolumn{1}{c}{Pro-R vs. Pro-D}&\multicolumn{1}{c}{Diff. by prior}\\
\hline
Climate topic   &    0.073&         0.058&         0.076\\
                    &  (0.009)&         (0.017)&       (0.007)  \\
Race topic          &    0.073&         0.031&         0.057\\
                    &  (0.019)&         (0.040)&       (0.008)  \\
Mobility topic      &    0.031&         0.037&         0.019\\
                    &  (0.005)&         (0.010)&       (0.005)  \\
Refugees topic      &    0.010&         0.016&         0.006\\
                    &  (0.002)&         (0.004)&       (0.001)  \\
Obama crime topic   &    0.026&         0.044&         0.010\\
                    &  (0.006)&         (0.012)&       (0.004)  \\
Gender topic        &    0.595&         0.511&         0.234\\
                    &  (0.182)&         (0.390)&       (0.129)  \\
Gun laws topic      &    0.002&         0.001&         0.001\\
                    &  (0.001)&         (0.002)&       (0.001)  \\
Media topic         &    0.000&         0.015&         0.018\\
                    &  (0.004)&         (0.009)&       (0.004)  \\
Rep score topic     &    0.028&         0.069&         0.022\\
                    &  (0.006)&         (0.014)&       (0.006)  \\
Dem score topic     &    0.032&         0.051&         0.024\\
                    &  (0.006)&         (0.013)&       (0.006)  \\
Own performance topic    &    0.007&         &         		0.013\\
               &  (0.003)&         &         		(0.003)\\
Question FE         &       No&      Yes&      Yes\\
\hline
Observations        &     8765&     7882&     8765\\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}


==> underperformance_overconfidence_gender-line.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    & News Pts         &                  &Performance         &                  &Expectation         &                  \\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\hline
Partisanship        &    -3.58\sym{***}&    -3.53\sym{***}&    -4.74\sym{*}  &    -4.89\sym{*}  &     6.13\sym{***}&     8.19\sym{***}\\
                    &   (1.13)         &   (1.15)         &   (2.60)         &   (2.68)         &   (2.18)         &   (2.16)         \\
Male                &                  &    -0.81         &                  &     3.65\sym{**} &                  &    11.98\sym{***}\\
                    &                  &   (0.71)         &                  &   (1.70)         &                  &   (1.31)         \\
Subject controls    &       No         &      Yes         &       No         &      Yes         &       No         &      Yes         \\
\hline
Observations        &     8696         &     8696         &      987         &      987         &      987         &      987         \\
\(R^{2}\)           &     0.00         &     0.00         &     0.00         &     0.04         &     0.01         &     0.13         \\
Mean                &    69.01         &    69.01         &    47.64         &    47.64         &    50.36         &    50.36         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> underperformance_overconfidence_no-gender.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    & News Pts         &                  &Performance         &                  &Expectation         &                  \\
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         \\
\hline
Partisanship        &    -3.58&    -3.53&    -4.74  &    -4.89  &     6.13&     8.19\\
                    &   (1.13)         &   (1.15)         &   (2.60)         &   (2.68)         &   (2.18)         &   (2.16)         \\
Subject controls    &       No         &      Yes         &       No         &      Yes         &       No         &      Yes         \\
\hline
Observations        &     8696         &     8696         &      987         &      987         &      987         &      987         \\
\(R^{2}\)           &     0.00         &     0.00         &     0.00         &     0.04         &     0.01         &     0.13         \\
Mean                &    69.01         &    69.01         &    47.64         &    47.64         &    50.36         &    50.36         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> wtp.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         \\
\hline
Assessment SD       &                  &   22.655&   22.605&   19.809 \\
                    &                  &  (8.421)         &  (8.470)         &  (8.688)         \\
Politicized topics  &    1.093         &                  &    1.052         &                  \\
                    &  (1.697)         &                  &  (1.701)         &                  \\
Constant            &    8.448&    4.234 &    3.466         &   10.504  \\
                    &  (1.498)         &  (2.078)         &  (2.436)         &  (5.968)         \\
Question FE         &       No         &       No         &       No         &      Yes         \\
Subject controls    &       No         &       No         &       No         &      Yes         \\
\hline
Observations        &      482         &      482         &      482         &      482         \\
\(R^{2}\)           &     0.00         &     0.02         &     0.02         &     0.06         \\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}
}


==> wtp_table.tex <==
\begin{tabular}{l*{4}{c}}
\hline\hline
                                   &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
\hline
Politicized Topic \hspace{30mm}                  &    0.572&         &    0.576&         \\
                                   &  (1.722)&         &  (1.723)&         \\
Assessment SD                      &         &   18.187&   18.190&   18.928\\
                                   &         &  (8.377)&  (8.403)&  (8.472)\\
Question FE                        &       No&       No&       No&      Yes\\
Subject controls                   &      Yes&      Yes&      Yes&      Yes\\
\hline
Observations                       &      482&      482&      482&      482\\
\(R^{2}\)                          &     0.03&     0.04&     0.04&     0.06\\
Mean                               &    9.257&    9.257&    9.257&    9.257\\
\hline\hline
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\end{tabular}

